End-to-End Imitation Learning with Safety Guarantees using Control Barrier Functions

Imitation learning (IL) is a learning paradigm which can be used to synthesize controllers for complex systems that mimic behavior demonstrated by an expert (user or control algorithm). Despite their popularity, IL methods generally lack guarantees of safety, which limits their utility for complex safety-critical systems. In this work we consider safety, formulated as set-invariance, and the associated formal guarantees endowed by Control Barrier Functions (CBFs). We develop conditions under which robustly-safe expert controllers, utilizing CBFs, can be used to learn end-to-end controllers (which we refer to as CBF-Compliant controllers) that have safety guarantees. These guarantees are presented from the perspective of input-to-state safety (ISSf) which considers safety in the context of disturbances, wherein it is shown that IL using robustly safe expert demonstrations results in ISSf with the disturbance directly related to properties of the learning problem. We demonstrate these safety guarantees in simulated vision-based end-to-end control of an inverted pendulum and a car driving on a track.

==> oldtext.tex <==


\section{Intro Notes}
Safety is of utmost importance for modern safety critical systems such as medical robots, autonomous vehicles, and human-assistive devices. By formalizing safety as the forward invariance of a safe set, several methods including model-predictive control, reachability methods, and control barrier functions are capable of generating provable safety guarantees for the system. 

Control Barrier Functions (CBFs )have become a popular tool for the constructive synthesis of model-based controllers. Originally described in \cite{ames_control_2017}, CBFs have been extended to retain their safety guarantees in the presence of dynamics uncertainty \cite{taylor_learning_nodate}, disturbances \cite{kolathaya2018input}, and measurement uncertainty \cite{dean_guaranteeing_2020}. 

End-to-End perception modules have also showed significant success in several situations such as pixel-to-torque of autonomous driving \cite{pan2017agile}. However, despite promising examples of performances, these methods lack guarantees of safety. 


CBFs \cite{ames_control_2017}

CBFs with learning \cite{taylor_learning_nodate, csomay-shanklin_episodic_nodate}

Perception with CBFs \cite{dean_guaranteeing_2020, cosner_measurement-robust_2021}

Learning CBFs from expert data \cite{robey_learning_2020}

Differentiable Optimization \cite{amos_optnet_nodate}

BarrierNet \cite{xiao_barriernet_2021}, Koushil's BarrierNet \cite{ma2022learning}

Differentiable QP Layers \cite{butler2021efficient} OptNet \cite{amos_optnet_nodate}

Dodgeball \cite{falanga_dynamic_2020-1, sanket_evdodgenet_2020, navarro_cassie_nodate}

MobileNet \cite{sandler2018mobilenetv2}

Power-Efficient Learning, Vivienne Sze \cite{noraky2017low} Journal version for rigid bodies \cite{noraky2019low}

End-to-end pixel to torque control \cite{pan2017agile}

NL-MPC dodgeball \cite{lindqvist2020nonlinear}

Exponential CBFs \cite{nguyen2016exponential}

Adversarially messing with the perception module \cite{boloor2020attacking}

Adversarial attacks for regressors \cite{nguyen2018adversarial}

tunable ISSf \cite{alan_safe_2022}

Imitation learning \cite{hussein2017imitation}

Safe Imitation Learning 
\begin{itemize}
    \item generalization robustness using RL and end-to-end imitation learning, learn uncertainty threshold using Bayesian neural networks. Bayesian models produce output prediction distributinos rather than point estimates which can be used for uncertainty estimation. Switching controller that compensates for high uncertainty from Bayesian NN \cite{lee2018safe}. \textit{Epistemic uncertainty} is when you lack data. \textit{Aleatoric uncertainty} inability to sense the entire state space from the inputs. 
    \item Imitation Learning, two methods: behavioral cloning (supervised learning) [Pomerleau 1991, Torabi 2018], suffers from compounding errors [Ross 2011] DAgger avois comdpounding errors by continuing to collect samples \cite{brown2020safe}. SafeDAgger and EnsembleDAgger, give control back to the expert when there is a large error prediction. \cite{brown2020safe} generates a high-confidence performance bound on robust policies. 
    \item Compounding errors in behavioral cloning (supervised learning) imitation learning \cite{ross2011reduction}. Traditional approach is supervised Learning .DAgger gets arround this by sampling states that the controller leads you too. That's not what we need! we benefit by the safe-set dimension reduction. 
    \item [Husseign survey paper], more sample efficient than reinforcement learning, more computationally efficient to evaluate online. Applications: video games, humanoids, selfdriving cars. Guarantees can come from Bayesian NNs, stability regualarization, or robust control \cite{tu2021closing}
    \item \cite{yin2021imitation} perhaps the closest to what we're doing in that they define safet yas set invariance of an ellipse. But it's limited to discrete time LTI systems. The force the unwrapped NN policy to respect certain constraints included what is essentially a discrete time barrier constraint. Discrete time linear systems. Use a "safe set" but it has to hace a very specific polytopic form. 
\end{itemize}


\cite{ross2010efficient} \cite{syed2010reduction}, time dependent deviation from expert trajectory. 


\clearpage

\section{Perception Notes}
In the rest of this work we adopt the following perception module. Consider the locally Lipschitz functions $\mb{c}: \R^n \to  \R^k$ and $\mb{k}_\theta:\R^k \to \R^m$. We assume that the function $\mb{c}$ maps from the system's state to a potentially high dimensional vector, such as a camera image. To generate a control input given the high dimensional vector $\mb{c}(\mb{x})$ we use the learned function $\mb{k}_\theta$ which, when inexact, generates the error: 
\begin{align}
    \mb{k}_\theta(\mb{c}(\mb{x})) -  \mb{k}_T(\mb{x})  =  \mb{e} (\mb{x}).
\end{align}
%  $\widehat{\mb{q}}_\theta: \R^k \to \R^n $ which attempts to map from images to states. This can be thought of as our perception function.
The learned end-to-end controller $\mb{k}_\theta$ is parameterized by the learned parameters $\theta$. 

\subsection{Imitation Learning}

In order to train the end-to-end controller $\mb{k}_\theta$, we collect a dataset of image-control input pairs:
\begin{align}
    D_i= (\mb{I}_i, \mb{k}_T(\mb{x})) \in \R^k \times \R^m  
\end{align}
whereby we can construct the training dataset $\mathcal{D} = \{ D_i \}^N_{i=1} $ for $N \in \mathbb{N}$ samples. Given a nonlinear function class $\mathcal{H}: \R^k \to \R^m $ and a loss function $\mathcal{L}: \R^m\times\R^m \to \R$, a learning problem can be specified as optimizing the parameters $\theta$ of the function $\mb{k}_\theta \in \mathcal{H}$ to estimate the empirical risk minimization: 
\begin{align}
    \min_{\mb{k}_\theta \in \mathcal{H}} \frac{1}{N} \sum_{i=1}^N \mathcal{L}\left( \mb{k}_\theta(\mb{I}_i), \mb{k}_T(\mb{x}_i) \right) 
\end{align}



\clearpage 



\clearpage 

\begin{proposition}
Let $\Omega: \R \rightsquigarrow \mathcal{P}(\R^n)$ map from $c\in \R$ to the $c$-superlevel set of a continuously differentiable function $h: \R^n \to \R$ and $\Omega(0) \subset \R^n  $ be compact and non-empty. If $0$ is a regular value of $h$ and for some $r_0>0 $ there exists a $\beta_0 > 0 $ such that $h(\mb{x}) \leq -\beta_0$ for all $\mb{x} \notin \Omega(0) \oplus B_{r_0} $, then $\Omega$ is upper semi-continuous at $0$.\label{prop:usc}
\end{proposition}

\begin{proof}
The set $\partial \Omega(0)$ is compact since it is a closed subset of the compact set $\Omega(0)$. Thus there exists a lower bound $\sigma \geq 0 $ such that $\min_{\mb{x} \in \partial \Omega(0) } \Vert \nabla h (\mb{x}) \Vert_2  = \sigma $. Since $h$ has 0 as a regular value, $\sigma$ must satisfy $\sigma > 0$.

Given $\varepsilon > 0 $, consider the expanded set $\Omega(0) \oplus \overline{B}_{\varepsilon}$. Note that $\Omega(0) \oplus \overline{B}_{\varepsilon}$ is compact since $\Omega(0) \times \overline{B}_{\varepsilon}$ is compact and $(\mb{x}, \mb{y}) \mapsto \mb{x}  + \mb{y} $ is continuous. 

Consider the state $\mb{x} \in (\Omega(0)\oplus\overline{B}_{\varepsilon'} )\setminus \Omega(0)$. There exists a $\mb{y} \in \partial \Omega (0) $ such that $\min_{\bs{\zeta} \in \Omega(0)  } \Vert  \mb{x} - \bs{\zeta} \Vert_2 = \Vert \mb{x} - \mb{y} \Vert_2 $. Since $h$ has 0 as a regular value, by \cite[Proposition 1.1.9]{clarke2008nonsmooth}, we have: 
\begin{align}
    \nabla h(\mb{y}) = - \Vert \nabla h (\mb{y}) \Vert_2 \frac{\mb{x} - \mb{y} }{\Vert \mb{x} - \mb{y} \Vert_2}.
\end{align}
\noindent Since $\overline{B}_{\varepsilon'}$ is convex, $\left(\lambda \mb{x} + (1-\lambda) \mb{y}\right) \in \Omega(0) \oplus \overline{B}_{\varepsilon'}$ for all $\lambda \in [0, 1] $. Additionally, for some $\lambda^* \in (0, 1) $, the state $\bs{\xi} \triangleq \lambda^*  \mb{x}  + (1 - \lambda^*) \mb{y} $ satisfies: 
\begin{align}
    h(\mb{x}) & = h(\mb{y}) + (\mb{x} - \mb{y})^\intercal\nabla h (\mb{y})  + \frac{1}{2}(\mb{x} - \mb{y})^\intercal \nabla^2 h(\bs{\xi}) (\mb{x} - \mb{y}).
\end{align}

Since $\Omega(0) \oplus \overline{B}_{\varepsilon'}$ is compact, there is an upper bound $\mu  \geq 0 $ such that $\max_{\mb{z} \in \Omega (0) \oplus \overline{B}_{\varepsilon'}} \Vert \nabla^2 h(\mb{z}) \Vert_2 = \mu $. We can use this to establish the following bound on $h$: 
\begin{align}
    h(\mb{x}) & \leq - \sigma \Vert \mb{x} - \mb{y} \Vert_2 + \frac{1}{\mu } \Vert \mb{x} - \mb{y} \Vert_2^2, \\
    & = - \left(\sigma - \frac{\mu}{2}\Vert \mb{x} - \mb{y}\Vert_2  \right)\Vert \mb{x} - \mb{y} \Vert_2.
\end{align}


If $\Vert \mb{x} - \mb{y} \Vert_2 \leq \sigma/\mu $, then the bound simplifies to
\begin{align}
    h(\mb{x}) \leq - \frac{\sigma}{2} \Vert \mb{x} - \mb{y} \Vert_2.  \label{eq:coercivity}
\end{align}

Choose $\varepsilon'> 0 $ such that $\varepsilon' < \min \{ \varepsilon, r_0, \sigma / \mu  \} $. The set $\partial\Omega(0) \oplus \overline{B}_{\varepsilon'}$ is compact so there is some $\beta_1 \in \R $ such that $-\beta_1 = \max_{\mb{z} \in \partial\Omega(0) \oplus \overline{B}_{\varepsilon'}} h(\mb{z})$. Additionally,  \eqref{eq:coercivity} implies that $\beta_1 \geq \sigma\varepsilon'/2  $.

Next, consider the band $\Gamma = (\Omega(0) \oplus \overline{B}_{r_0}) \setminus (\Omega(0) \oplus B_{\varepsilon'}) $ which can be written equivalently as $(\Omega(0) \oplus \overline{B}_{r_0}) \cap (\Omega(0) \oplus B_{\varepsilon'})^C$. Since $\Gamma$ is the intersection of a compact and closed set, $\Gamma $ is compact. Since $\varepsilon' < r_0$ and $\Omega(0) $ is non-empty, $\Gamma $ is non-empty. $\Gamma$ is compact and non-empty so there is a bound $\beta_2\in \R$ such that 
$- \beta_2 =  \max_{\mb{z} \in \Gamma} h(\mb{z}) $. This bound is greater than zero $\beta_2>0$ since $\Gamma \cap \Omega(0) = \emptyset $

Thus $h(\mb{x}) \leq \max \{ -\beta_0, -\beta_2 \}  <  0$ for all $\mb{x} \in \R^n \setminus (\Omega(0) \oplus B_{\varepsilon'})$. 
Choose $\eta < \beta_2$, this ensures that $\mb{x} \in \Omega(-\eta) \implies  $\mb{x} \in \Omega(0) \oplus \overline{B}_{\varepsilon'}$. Since a superlevel set contains all superlevel sets of greater value, $\Omega(-\eta) \subseteq \Omega(0)\oplus B_{\varepsilon'}$ ensures that $c \in (\eta, -\eta ) \implies \Omega(c) \subseteq \Omega(0) \oplus B_{\varepsilon'}$ and thus $\Omega$ is upper semi-continuous. 

%Choose $\eta < \min \{ \beta_2, \sigma/2\varepsilon' \} $, $\eta < \beta_2$ ensures that $\mb{x} \in \Omega(\eta) \implies \mb{x} \in \Omega(0) \oplus \overline{B}_{\varepsilon'}$ and $\eta < \sigma/2 \varepsilon'$

One example of a safe set that satisfies the conditions of this proposition is the inverted ellipse: $h(\mb{x}) = c - \mb{x}^\intercal \mb{P} \mb{x} $ where $c > 0 $ and $\mb{P}\in\mathbb{S}_{>0}$.

% \begin{proof}
% By andrew's proof we reach $h(\mb{x}) \leq -\frac{\sigma}{2} \Vert \mb{x} - \mb{y} \Vert $ for $\mb{x} \notin \mathcal{C} \oplus B_\epsilon$. Stitch this with the assumption that $\mathcal{X}$ is compact and there is a maximum $-\beta $ achieved outside of the set.  Since $\mathcal{X} $ is compact and $\mathcal{C} \oplus B_{\epsilon}$ is open,  $\mathcal{X} \setminus (\mathcal{C} \oplus B_{\epsilon})$ is compact, thus $-\beta = \max_{\mb{x} \not \in \mathcal{X} \setminus (\mathcal{C} \oplus B_{\epsilon})} h ( \mb{x})$ for some $ \beta > 0 $. By choosing $\epsilon' $ such that $-N \epsilon' > -\beta $, then $\Omega (-N\epsilon') \subset \mathcal{C}\oplus B_{\epsilon'}$. 

% Let $\delta = N\epsilon' < N \epsilon$, then for any $\epsilon>0$, $c \in B_{\delta} \implies \Omega(c) \subset \mathcal{C} \oplus B_\epsilon $ since $\Omega(-N\epsilon') \subset \mathcal{C} \oplus B_\epsilon $ and the superlevel set $\Omega(-N\epsilon')$ contains all superlevel sets $\Omega (c') $ where $c' > 0 $. Thus $\Omega$ is upper semi-continuous at $0 $. 
% \end{proof}

% \begin{proof}
% The set $\mathcal{C}$ is a compact, so its boundary $\partial \mathcal{C}$ is also compact. $h$ has 0 as a regular value so $\min_{\mb{x} \in \partial \mathcal{C}} \frac{\partial h}{\partial \mb{x} }\vert_{\mb{x}} = -M < 0 $ is achieved for some $\mb{x}^* \in \partial \mathcal{C}$. 

% Since $\frac{\partial h}{\partial \mb{x}}$ is continuous, for any $N < M$, there exists some $\epsilon > 0 $ such that $\min_{\mb{x} \in \partial \mathcal{C}\oplus B_{\epsilon}} \frac{\partial h }{\partial x} = - N < 0 $ is achieved by some $\mb{x}^* \in \partial \mathcal{C}\oplus B_{\epsilon} $.

% For all $\mb{x} \in \mathcal{C} \setminus (\partial \mathcal{C}\oplus B_{\epsilon'})$ and $\mb{y}$ be a point such that $\mb{y} = \min_{\mb{y} \in \partial \mathcal{C}} \Vert \mb{x} = \mb{y} \Vert$; $\mb{y}$ exists since $\partial \mathcal{C}$ is compact. This construction can be used to upper bound $h(\mb{x})$  
% \begin{align}
%     h(\mb{x})  = h(\mb{x} + \mb{y} -\mb{y} ) &\leq h(\mb{y}) - N \Vert \mb{x}  \Vert_\mathcal{C} = - N \Vert \mb{x} \Vert_\mathcal{C}, 
% \end{align}
% so $h(\mb{x}) < - N \epsilon' $. Since $\mathcal{X} $ is compact and $\mathcal{C} \oplus B_{\epsilon}$ is open,  $\mathcal{X} \setminus (\mathcal{C} \oplus B_{\epsilon})$ is compact, thus $-\beta = \max_{\mb{x} \not \in \mathcal{X} \setminus (\mathcal{C} \oplus B_{\epsilon})} h ( \mb{x})$ for some $ \beta > 0 $. By choosing $\epsilon' $ such that $-N \epsilon' > -\beta $, then $\Omega (-N\epsilon') \subset \mathcal{C}\oplus B_{\epsilon'}$. 

% Let $\delta = N\epsilon' < N \epsilon$, then for any $\epsilon>0$, $c \in B_{\delta} \implies \Omega(c) \subset \mathcal{C} \oplus B_\epsilon $ since $\Omega(-N\epsilon') \subset \mathcal{C} \oplus B_\epsilon $ and the superlevel set $\Omega(-N\epsilon')$ contains all superlevel sets $\Omega (c') $ where $c' > 0 $. Thus $\Omega$ is upper semi-continuous at $0 $. 

% \end{proof}

% We note that the assumption of compactness for $\mathcal{X}$ can be removed if $\sup_{\mb{x} \in \mathcal{X}\setminus (\mathcal{C}\oplus B_\epsilon )} < 0 $. 

% The proof of Proposition \ref{prop:usc} follows the structure presented in  \cite{taylor2022sdcbf} and is included below for completeness. 


% \begin{proof}

% \textcolor{blue}{
% $h$ has 0 as a regular value and $\mathcal{C}$ is compact so $\partial \mathcal{C}$ is compact and there exists some $M >0 $ such that $\min_{\mb{x} \in \partial \mathcal{C}} \Vert \frac{\partial h}{\partial\mb{x}}(\mb{x}) \Vert \geq M$. $h $ is continuously differentiable, so $dh/d\mb{x} $ is continuous, so for any $\epsilon $  where $M > \epsilon >0 $ there exists an $\delta > 0 $ such that for all $\mb{x} \in \partial \mathcal{C} \oplus B_\epsilon $ it is true that $\min_{\mb{x} }\Vert dh/d\mb{x}\Vert > \delta$.
% So $h(\mb{x}) = h(\mb{x} + - \mb{y}) \geq h(\mb{y} \in \mathcal{C}) - \delta \Vert \mb{x} - \mb{y} \Vert   = - \delta \Vert \mb{x} - \mb{y} \Vert$ (using lipschitz and regular value to say that lipschitz cannot be zero). Since the closed expansion of 
% }

% Consider a real valued sequence $\{ c_n \in \R ~|~ n \in \mathbb{N} \} $ converging to $0$ and a state-valued sequence $\{ \mb{x}_n \in \R^n ~|~ n \in \mathbb{N}\}$ with $\mb{x}_n \in \Omega(c_n) $. For any $\varepsilon'>0$ with $0 + \varepsilon' < c^* $, there is a corresponding $N_{\varepsilon'}\in \mathbb{N}$ such that $|0 - c_n | < \varepsilon'$ for all $n \in \mathbb{N}$ with $n \geq \mathbb{N}_{\varepsilon'}$. This means that 
% \begin{align}
%     h(\mb{x}_n) \leq 0 + \varepsilon' < c^* 
% \end{align}
% or $\mb{x}_n \in \Omega (c^*) $ for all $n \in \mathbb{N} $ with $n \geq N_{\varepsilon'}$. Since $\Omega(c^*)$ is compact, there is a state-valued subsequence converging to a limit in $\Omega (c^*) $; denote this subsequence by $\{\mb{x}_{n_k} ~|~ k \in \mathbb{N } \} $ and denote its limit by $ \mb{x} \in \Omega(c^*) $. For any $\varepsilon' >0 $ there is a corresponding $K_{\varepsilon'}\in \mathbb{N}$ such that 
% \begin{align}
%     h(\mb{x}_{n_k})\leq 0 + \varepsilon'
% \end{align}
% for all $k \in \mathbb{N}$ with $k \geq K_{\varepsilon'}$. Since $\varepsilon'$ was arbitrary and $h$ is continuous, $h(\mb{x}) \leq 0 $ or $\mb{x} \in \Omega(0)$. Thus $\Omega$ is upper semi-continuous by the second equivalent condition and must therefore also satisfy the first. 
% \end{proof} 
% \textcolor{blue}{TODO: Must show that regular value implies the existence of a $c^* < 0 $ such that the superlevel set is compact. }


==> reviewer_comments.tex <==
Associate Editor:
